BenX: Resource-Sharing Permutations for Computational Integrity

Cryptographic hash functions over integers modulo a prime play a decisive role in the efficiency and security of proof systems for computational integrity. Early designs focused on compact arithmetic circuits and efficient software execution, primarily targeting general-purpose CPUs rather than hardware accelerators. This work focuses on enabling efficient resource sharing and hardware acceleration alongside efficient software execution. We propose BenX, a permutation-based hash function designed for hardware acceleration, fast CPU execution, and low circuit complexity in proof systems. To construct the underlying permutation, we turn the Benes network into an invertible function over $\mathbb{F}_p^2$ using a Dickson polynomial. Its structure yields a permutation particularly suited to hardware resource sharing and acceleration. Fully pipelined on FPGA, BenX matches the throughput of Poseidon2, with 1.36x and 2.15x lower latency for Goldilocks and BabyBear, respectively. Although larger as a standalone core, it makes more effective use of shared hardware: in our dual-mode architecture, where the NTT and hash share field multipliers, BenX keeps 100% of them busy, compared with 6.25-20.3% for the partial rounds of Poseidon and Poseidon2. In software, BenX outperforms Poseidon in all tested 31- and 64-bit configurations, but is slower than Poseidon2, except for the 16-element BabyBear instance. In zero-knowledge proofs, BenX proves Goldilocks permutations 6-10x faster than Monolith. Its compact arithmetization uses about 36% fewer trace cells than Poseidon and Poseidon2 over BabyBear, while its fast variant requires 1.3-2.6x the prover time of Poseidon2.

==> tikzlibrarycipher.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% TIKZLIBRARY CIPHER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Utilities for drawing cryptographic circuits                               %
%   Version: 2018-10-01                                                        %
%   Author: Maria Eichlseder                                                   %
%   \usetikzlibrary{cipher}                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SHAPES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% UTILS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% from https://tex.stackexchange.com/questions/14769/add-more-anchors-to-standard-tikz-nodes
\newcommand{\anchorlet}[2]{%
    \global\expandafter
    \let\csname pgf@anchor@\pgf@sm@shape@name @#1\expandafter\endcsname
    \csname pgf@anchor@\pgf@sm@shape@name @#2\endcsname
}

%%% OPERATION SHAPES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{oplus}{%{{{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \foreach \s in {center,mid,base,text, north,south,west,east,
                  mid west,mid east,base west,base east,
                  north west,south west,north east,south east} {
    \inheritanchor[from=circle]{\s}
  }
  %\inheritbackgroundpath[from=circle]
  % From /usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex:1148
  \backgroundpath{%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
    % north-south
    \centerpoint\advance\pgf@y by\radius  \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \centerpoint\advance\pgf@y by-\radius \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    % east-west
    \centerpoint\advance\pgf@x by\radius  \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \centerpoint\advance\pgf@x by-\radius \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}%}}}

\pgfdeclareshape{ominus}{%{{{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \foreach \s in {center,mid,base,text, north,south,west,east,
                  mid west,mid east,base west,base east,
                  north west,south west,north east,south east} {
    \inheritanchor[from=circle]{\s}
  }
  %\inheritbackgroundpath[from=circle]
  % From /usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex:1148
  \backgroundpath{%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
    % east-west
    \centerpoint\advance\pgf@x by\radius  \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \centerpoint\advance\pgf@x by-\radius \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}%}}}

\pgfdeclareshape{otimes}{%{{{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \foreach \s in {center,mid,base,text, north,south,west,east,
                  mid west,mid east,base west,base east,
                  north west,south west,north east,south east} {
    \inheritanchor[from=circle]{\s}
  }
  %\inheritbackgroundpath[from=circle]
  % From /usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex:1148
  \backgroundpath{%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
    % nw-se
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc  \pgf@xa=\pgf@x 
    \advance\pgf@y by 0.707107\pgf@xc  \pgf@ya=\pgf@y
    \centerpoint
    \advance\pgf@x by 0.707107\pgf@xc  \pgf@xb=\pgf@x 
    \advance\pgf@y by-0.707107\pgf@xc  \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    % sw-ne
    \centerpoint
    \advance\pgf@x by-0.707107\pgf@xc  \pgf@xa=\pgf@x 
    \advance\pgf@y by-0.707107\pgf@xc  \pgf@ya=\pgf@y
    \centerpoint
    \advance\pgf@x by 0.707107\pgf@xc  \pgf@xb=\pgf@x 
    \advance\pgf@y by 0.707107\pgf@xc  \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}%}}}

\pgfdeclareshape{boxplus}{%{{{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \foreach \s in {center,mid,base,text, north,south,west,east,
                  mid west,mid east,base west,base east,
                  north west,south west,north east,south east} {
    \inheritanchor[from=rectangle]{\s}
  }
  \backgroundpath{
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    % store center in xc/yc
    \pgf@xc=.5\pgf@xa \advance\pgf@xc by .5\pgf@xb
    \pgf@yc=.5\pgf@ya \advance\pgf@yc by .5\pgf@yb
    % construct main path
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
    \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
  }
}%}}}

%%% PRIMITIVE SHAPES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{compressionf}{%{{{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]

  \foreach \s in {center,base,text,
                  north,south,west,east,
                  north west, south west, north east, south east} {
    \inheritanchor[from=rectangle]{\s}
  }
  \anchor{msg}{\southwest \pgf@xa=\pgf@x 
               \northeast \pgf@x=\pgf@xa}
  \anchor{tip}{\southwest \pgf@xa=\pgf@x
               \northeast
               \pgf@x=\pgf@xa
               \advance\pgf@y by \pgf@y}
  \anchor{top}{\southwest \pgf@xa=\pgf@x
               \northeast 
               \advance\pgf@x by-.5\pgf@x
               \advance\pgf@x by .5\pgf@xa
               \advance\pgf@y by .5\pgf@y}
  \backgroundpath{
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@xa
    \pgf@yc=\pgf@yb \advance\pgf@yc by \pgf@yb

    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
  }
}%}}}

\pgfdeclareshape{compression}{%{{{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]

  \foreach \s in {center,base,text,
    north,south,west,east,
    north west, south west, north east, south east} {
    \inheritanchor[from=rectangle]{\s}
  }
  \backgroundpath{
    % store lower left in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@xa \advance\pgf@xc by .75\pgf@xa
    \pgf@yc=\pgf@xb \advance\pgf@yc by-.75\pgf@xa

    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
  }
}%}}}

\pgfdeclareshape{filter}{%{{{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]

  \foreach \s in {center,base,text,
                  north,south,west,east,
                  north west, south west, north east, south east} {
    \inheritanchor[from=rectangle]{\s}
  }
  \backgroundpath{
    % store lower left in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@xa \advance\pgf@xc by .75\pgf@xa
    \pgf@yc=\pgf@xb \advance\pgf@yc by-.75\pgf@xa

    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
  }
}%}}}

\pgfdeclareshape{authentication}{%{{{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]

  \foreach \s in {center,base,text,
                  north,south,west,east,
                  north west, south west, north east, south east} {
    \inheritanchor[from=rectangle]{\s}
  }
  \anchor{tag}{\northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               %\southwest \pgf@x=\pgf@xa}
               \southwest \pgf@x=\pgf@xa \advance\pgf@y by .5\pgf@y \advance\pgf@y by -.5\pgf@ya}
  \anchor{tip}{\northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \southwest
               \pgf@x=\pgf@xa
               %\advance\pgf@y by \pgf@y}
               \advance\pgf@y by \pgf@y \advance\pgf@y by -\pgf@ya}
  \anchor{bot}{\northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \southwest 
               \advance\pgf@x by-.5\pgf@x
               \advance\pgf@x by .5\pgf@xa
               %\advance\pgf@y by .5\pgf@y}
               \advance\pgf@y by .5\pgf@y \advance\pgf@y by -.5\pgf@ya}
  \backgroundpath{
    % store upper right in xa/ya and lower left in xb/yb
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@xa
    %\pgf@yc=\pgf@yb \advance\pgf@yc by \pgf@yb
    \pgf@yc=\pgf@yb \advance\pgf@yc by \pgf@yb \advance\pgf@yc by -\pgf@ya

    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
  }
}%}}}

\pgfdeclareshape{wide}{%{{{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]

  \foreach \s in {center,base,text,
                  north,south,west,east,
                  north west, south west, north east, south east} {
    \inheritanchor[from=rectangle]{\s}
  }
  \anchor{wnw}{\northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \southwest \advance\pgf@y by-.75\pgf@y
                          \advance\pgf@y by .75\pgf@ya}
  \anchor{wsw}{\northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \southwest \advance\pgf@y by-.25\pgf@y
                          \advance\pgf@y by .25\pgf@ya}
  \anchor{ene}{\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \northeast \advance\pgf@y by-.25\pgf@y
                          \advance\pgf@y by .25\pgf@ya}
  \anchor{ese}{\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \northeast \advance\pgf@y by-.75\pgf@y
                          \advance\pgf@y by .75\pgf@ya}

  \anchor{nnw}{\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \northeast \advance\pgf@x by-.75\pgf@x
                          \advance\pgf@x by .75\pgf@xa}
  \anchor{nne}{\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \northeast \advance\pgf@x by-.25\pgf@x
                          \advance\pgf@x by .25\pgf@xa}
  \anchor{ssw}{\northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \southwest \advance\pgf@x by-.25\pgf@x
                          \advance\pgf@x by .25\pgf@xa}
  \anchor{sse}{\northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
               \southwest \advance\pgf@x by-.75\pgf@x
                          \advance\pgf@x by .75\pgf@xa}

  \inheritbackgroundpath[from=rectangle]

  \anchorlet{xouter}{wnw}
  \anchorlet{youter}{ene}
  \anchorlet{xinner}{wsw}
  \anchorlet{yinner}{ese}
}%}}}

% TODO keyed north/west/south/east

%%% OTHER SHAPES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{document}{%{{{
  % paper with folded corner
  % from PGF manual, "Command for Declare New Shapes"
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \backgroundpath{
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    % compute corner of ‘‘flipped page’’
    \pgf@xc=\pgf@xb \advance\pgf@xc by-5pt % this should be a parameter
    \pgf@yc=\pgf@yb \advance\pgf@yc by-5pt
    % construct main path
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
    % add little corner
    \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
  }
}
\pgfdeclareshape{minidocument}{
  % paper with folded corner
  % from PGF manual, "Command for Declare New Shapes"
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \backgroundpath{
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    % compute corner of ‘‘flipped page’’
    \pgf@xc=\pgf@xb \advance\pgf@xc by-2pt % this should be a parameter
    \pgf@yc=\pgf@yb \advance\pgf@yc by-2pt
    % construct main path
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
    % add little corner
    \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
  }
}
\tikzset{doc/.style={draw, fill=none, shape=document}}
\tikzset{minidoc/.style={draw, fill=none, shape=minidocument}}
%}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% MATRIX STATE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\State}[1]{%
  \tikz[stateopts]{
    \foreach \x/\y/\s in {0/0/0, 0/1/1, 0/2/2, 0/3/3,
                          1/0/4, 1/1/5, 1/2/6, 1/3/7,
                          2/0/8, 2/1/9, 2/2/10,2/3/11,
                          3/0/12,3/1/13,3/2/14,3/3/15} {
       %
      \draw (\y+.5,-\x-.5) coordinate (s\s) coordinate (ss\x\y); % (rowwise indices)
      \draw (\x+.5,-\y-.5) coordinate (b\s); % AES indices (columnwise)
    }
    #1
    \draw (0,0) rectangle (4,-4);
    \foreach \x in {1,2,3} {
      \draw[raster] (0,-\x) -- ++(4,0);
      \draw[raster] (\x,0) -- ++(0,-4);
    }
  }%
}
\newcommand{\Column}[1]{%
  \tikz[stateopts]{
    \foreach \x/\y/\s in {0/0/0, 1/0/4, 2/0/8, 3/0/12} {
      \draw (\y+.5,-\x-.5) coordinate (s\s) coordinate (ss\x\y); % (rowwise indices)
    }
    #1
    \draw (0,0) rectangle (1,-4);
    \foreach \x in {1,2,3} { \draw[raster] (0,-\x) -- ++(1,0); }
  }%
}

\newcommand{\Cell}[2]{\draw (#1) node[inner sep=0pt,cellopts] {#2\vphantom{0}};}
\newcommand{\FillCell}[2][fillopts]{\fill[#1] (#2) ++(-.5,.5) rectangle +(1,-1);}
\newcommand{\Fill}[2][fillopts]{\FillCell[#1]{#2}}
\newcommand{\FillColumn}[2][fillopts]{\fill[#1] (ss0#2) ++(-.5,.5) rectangle +(1,-4);}
\newcommand{\FillDiagonal}[2][fillopts]{\foreach \dd in {0,...,3} {\pgfmathsetmacro{\dx}{mod(int(\dd)+int(#2),4)}\Fill[#1]{ss\dd\dx}}}
\newcommand{\FillAntiDiagonal}[2][fillopts]{\foreach \dd in {0,...,3} {\pgfmathsetmacro{\dx}{mod(int(#2)+4-int(\dd),4)}\Fill[#1]{ss\dd\dx}}}
\newcommand{\FillState}[1][fillopts]{\fill[#1] (0,0) rectangle (4,-4);}

% TODO check out if TiKZ matrices (tikzmanual.pdf Chapter 20) could be useful instead

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ARROWS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{arrows.meta}
\pgfarrowsdeclare{ipe arrow}{ipe arrow}{%{{{
  \pgfutil@tempdima=5pt\relax
  \advance\pgfutil@tempdima-1.5\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{1.5\pgflinewidth}{0pt}}%
  \pgfpathmoveto{\pgfpointorigin}%
  \pgfpathlineto{\pgfqpoint{-5pt}{-1.666pt}}%
  \pgfpathlineto{\pgfqpoint{-5pt}{+1.666pt}}%
  \pgfpathclose
  \pgfusepathqfill
}%}}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% STYLES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% OPERATION STYLES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{op/.style={draw, fill=none, minimum size=1.5ex, inner sep=0pt}}
\tikzset{xor/.style={op, shape=oplus}}
\tikzset{not/.style={op, shape=ominus}}
\tikzset{mul/.style={op, shape=otimes}}
\tikzset{and/.style={op, shape=otimes}} % TODO \odot
\tikzset{sum/.style={op, shape=boxplus}}
\tikzset{tee/.style={shape=circle, fill, draw, inner sep=0pt, minimum size=2pt}}
\tikzset{rot/.style={shape=rectangle, draw, inner sep=2pt, rounded corners=2pt}} % TODO

%%% PRIMITIVE STYLES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{box/.style={minimum size=.75cm, draw, inner sep=1pt, fill=white, rounded corners=3pt}}

\tikzset{
  key west/.style={path picture={\draw[line cap=round,rounded corners=0pt] (path picture bounding box.west) +(.25pt,.65ex) -- +(.65ex,0) -- +(.25pt,-.65ex);}},
  key east/.style={path picture={\draw[line cap=round,rounded corners=0pt] (path picture bounding box.east) +(-.25pt,.65ex) -- +(-.65ex,0) -- +(-.25pt,-.65ex);}},
  key north/.style={path picture={\draw[line cap=round,rounded corners=0pt] (path picture bounding box.north) +(-.65ex,-.25pt) -- +(0,-.65ex) -- +(.65ex,-.25pt);}},
  key south/.style={path picture={\draw[line cap=round,rounded corners=0pt] (path picture bounding box.south) +(-.65ex,.25pt) -- +(0,.65ex) -- +(.65ex,.25pt);}},
  key at/.style args = {#1}{path picture={\draw[line cap=round,rounded corners=0pt] (path picture bounding box.#1) +(-.65ex,.25pt) -- +(0,.65ex) -- +(.65ex,.25pt);}},
}

%%% ARROW STYLES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{next/.style={->, >=ipe arrow}}
\tikzset{prev/.style={<-, >=ipe arrow}}

%%% MATRIX STATE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{
  state/.style={inner sep=0pt},
  stateopts/.style={scale=.3},
  raster/.style={},
  fillopts/.style={gray},
  cellopts/.style={},
}

% TODO provide settings that prefill nodes with \State{}

% TODO alternative shapes -- careful, they mess up with chained comments and relative coordinates!
\tikzset{
  notalt/.style={draw,circle,append after command={
                 [shorten >=\pgflinewidth, shorten <=\pgflinewidth]
                 (\tikzlastnode.east) edge (\tikzlastnode.west)
                }},
  xoralt/.style={draw,circle,append after command={
                 [shorten >=\pgflinewidth, shorten <=\pgflinewidth]
                 (\tikzlastnode.north) edge (\tikzlastnode.south)
                 (\tikzlastnode.east) edge (\tikzlastnode.west)
                }},
  andalt/.style={op, shape=circle, node contents={\tikz{\filldraw circle (.75pt);}} },
}

% vim: foldmethod=marker

